Multi-wavelength Observations of 3C 273 in 1993-1995

We present the results of the multi-wavelength campaigns on 3C 273 in 1993-1995. During the observations in late 1993 this quasar showed an increase of its flux for energies greater equal 100 MeV from about 2.1 x 10^-7 photons/cm^2/s to approximately 5.6 x 10^-7 photons/cm^2/s during a radio outburst at 14.5, 22 and 37 GHz. However, no one-to-one correlation of the gamma-ray radiation with any frequency could be found. The photon spectral index of the high energy spectrum changed from (3.20 +- 0.54) to (2.20 +- 0.22) in the sense that the spectrum flattened when the gamma-ray flux increased. Fits of the three most prominent models (synchrotron self-Comptonization, external inverse Comptonization and the proton initiated cascade model) for the explanation of the high gamma-ray emission of active galactic nuclei were performed to the multi-wavelength spectrum of 3C 273. All three models are able to represent the basic features of the multi-wavelength spectrum. Although there are some differences the data are still not decisive enough to discriminate between the models.

==> tab3.tex <==
%auto-ignore
\begin{table}[ht]
\bigskip
\centerline{
\begin{tabular}{ccccccc}
\hline\hline
MJD&\multispan2   2.7GHz &\multispan2   4.75GHz   &\multispan2 10.55GHz  \\
   &Flux(Jy)&$\sigma$(Jy)&Flux(Jy)&$\sigma$(Jy)&Flux(Jy)&$\sigma$(Jy)\\
\noalign{\hrule}
48335 & ...   &  ...  & 33.40 &  0.50 & ...   &  ...  \\
48536 & 42.10 &  3.00 & 33.90 &  0.70 & 44.00 &  2.50 \\
48567 & 37.10 &  0.60 & 34.00 &  0.70 & ...   &  ...  \\
48588 & 39.40 &  1.70 & 35.20 &  1.20 & 45.70 &  1.20 \\
48602 & 41.50 &  1.00 & 35.60 &  0.40 & 43.50 &  2.20 \\
48673 & 40.00 &  2.70 & 36.50 &  1.50 & 44.90 &  3.00 \\
48685 & 38.70 &  2.90 & ...   &  ...  & 45.70 &  4.80 \\
48726 & 39.30 &  1.00 & ...   &  ...  & 47.10 &  2.50 \\
48741 & 38.90 &  1.10 & 36.70 &  1.30 & 46.90 &  2.90 \\
48775 & 41.70 &  1.60 & 39.80 &  1.80 & 46.50 &  2.30 \\
48799 & 40.40 &  2.20 & ...   &  ...  & 43.30 &  4.00 \\
48819 & ...   &  ...  & ...   &  ...  & 47.00 &  1.00 \\
48883 & ...   &  ...  & ...   &  ...  & 45.00 &  1.00 \\
48904 & 40.80 &  1.50 & ...   &  ...  & 44.80 &  1.00 \\
48966 & 40.00 &  1.30 & 40.60 &  1.50 & 43.00 &  2.00 \\
48967 & ...   &  ...  & ...   &  ...  & 44.80 &  2.00 \\
48996 & 41.70 &  1.80 & 42.00 &  1.40 & 43.90 &  1.00 \\
48997 & 42.20 &  1.60 & 41.60 &  1.40 & 45.60 &  2.20 \\
49027 & 41.90 &  1.60 & 41.90 &  2.20 & 44.80 &  2.70 \\
49056 & ...   &  ...  & ...   &  ...  & 43.40 &  2.20 \\
49071 & 43.20 &  1.70 & 42.40 &  1.90 & 43.00 &  2.40 \\
49108 & 42.30 &  1.70 & 43.00 &  2.30 & 41.10 &  1.50 \\
49158 & ...   &  ...  & 43.20 &  1.30 & 41.70 &  1.50 \\
49184 & 42.80 &  1.10 & ...   &  ...  & ...   &  ...  \\
49185 & 42.80 &  1.20 & 43.20 &  1.80 & 41.40 &  1.50 \\
49217 & 43.60 &  1.50 & 43.80 &  1.80 & ...   &  ...  \\
49218 & 43.00 &  1.50 & ...   &  ...  & ...   &  ...  \\
49219 & 45.90 &  1.70 & ...   &  ...  & 40.50 &  2.00 \\
49297 & 45.70 &  2.10 & 41.60 &  1.70 & 40.90 &  2.70 \\
49299 & ...   &  ...  & 43.10 &  1.70 & 39.30 &  2.10 \\
49332 & 44.80 &  1.40 & ...   &  ...  & ...   &  ...  \\
49349 & 44.80 &  1.70 & 42.70 &  1.60 & 39.80 &  1.60 \\
49381 & 45.00 &  1.40 & 42.30 &  1.20 & 40.30 &  1.90 \\
49413 & 44.70 &  1.60 & 42.80 &  1.60 & 39.70 &  1.80 \\
49430 & 44.30 &  1.60 & 43.40 &  1.60 & 41.50 &  2.00 \\
49713 & 46.30 &  2.60 & 43.00 &  2.50 & ...   &  ...  \\
49756 & 45.90 &  1.90 & 41.10 &  1.30 & ...   &  ...  \\
\end{tabular}
}
\end{table}
